A Lower Bound on the Error Exponent of Linear Block Codes over the Erasure Channel

A lower bound on the maximum likelihood (ML) decoding error exponent of linear block code ensembles, on the erasure channel, is developed. The lower bound turns to be positive, over an ensemble specific interval of erasure probabilities, when the ensemble weight spectral shape function tends to a negative value as the fractional codeword weight tends to zero. For these ensembles we can therefore lower bound the block-wise ML decoding threshold. Two examples are presented, namely, linear random parity-check codes and fixed-rate Raptor codes with linear random precoders. While for the former a full analytical solution is possible, for the latter we can lower bound the ML decoding threshold on the erasure channel by simply solving a 2 x 2 system of nonlinear equations.

==> tex/acronyms2.tex <==
% A
\DeclareAcronym{AWGN}{short = AWGN ,long = additive white gaussian noise}
\DeclareAcronym{ACRDA}{short = ACRDA ,long = asynchronous contention resolution diversity ALOHA}
% B
% C
\DeclareAcronym{CDF}{short = CDF ,long = cumulative distribution function}
\DeclareAcronym{CRA-CC}{short = CRA-CC ,long = CRA-convolutional code}
\DeclareAcronym{CRA-SH}{short = CRA-SH ,long = CRA-shannon bound}
\DeclareAcronym{CRA}{short = CRA ,long = contention resolution ALOHA}
\DeclareAcronym{CRDSA}{short = CRDSA ,long = contention resolution diversity slotted ALOHA}
\DeclareAcronym{CRDSA++}{short = CRDSA++ ,long = contention resolution diversity slotted ALOHA++}
\DeclareAcronym{CSA}{short = CSA ,long = coded slotted ALOHA}
% D
\DeclareAcronym{DAMA}{short = DAMA ,long = demand assigned multiple access}
\DeclareAcronym{DSA}{short = DSA ,long = diversity slotted ALOHA}
% E
\DeclareAcronym{ECRA}{short = ECRA ,long = enhanced contention resolution ALOHA}
\DeclareAcronym{ECRA-SC}{short = ECRA-SC ,long = ECRA selection combining}
\DeclareAcronym{ECRA-MRC}{short = ECRA-MRC ,long = ECRA maximal-ratio combining}
\DeclareAcronym{EGD}{short = EGD ,long = equal-gain diversity}
% F
\DeclareAcronym{FEC}{short = FEC ,long = forward error correction}
% G
\DeclareAcronym{GEO}{short = GEO ,long = geostationary orbit}
% H
% I
\DeclareAcronym{IC}{short = IC ,long = interference cancellation}
\DeclareAcronym{IRCRA}{short = IRCRA ,long = irregular repetition contention resolution ALOHA}
\DeclareAcronym{IRSA}{short = IRSA ,long = irregular repetition slotted ALOHA}
% K
% L
% M
\DeclareAcronym{M2M}{short = M2M ,long = machine-to-machine}
\DeclareAcronym{MAC}{short = MAC ,long = medium access}
\DeclareAcronym{MF-TDMA}{short = MF-TDMA ,long = multi-frequency time division multiple access}
\DeclareAcronym{MRC}{short = MRC ,long = maximal-ratio combining}
% N
% O
% P
\DeclareAcronym{PDF}{short = PDF ,long = probability density function}
\DeclareAcronym{PER}{short = PER ,long = packet error rate}
\DeclareAcronym{PLR}{short = PLR ,long = packet loss rate}
% Q
% R
\DeclareAcronym{RA}{short = RA ,long = random access}
\DeclareAcronym{RCB}{short = RCB ,long = random coding bound}
\DeclareAcronym{RTT}{short = RTT ,long = round trip time}
% S
\DeclareAcronym{SA}{short = SA , long = slotted ALOHA}
\DeclareAcronym{SB}{short = SB ,long = Shannon bound}
\DeclareAcronym{SC}{short = SC ,long = selection combining}
\DeclareAcronym{SIC}{short = SIC ,long = successive interference cancellation}
\DeclareAcronym{SNIR}{short = SNIR ,long = signal-to-noise and interference ratio}
\DeclareAcronym{SINR}{short = SINR ,long = signal-to-interference and noise ratio}
\DeclareAcronym{SNR}{short = SNR ,long = signal-to-noise ratio}
% T
\DeclareAcronym{TDMA}{short = TDMA ,long = time division multiple access}
% U
\DeclareAcronym{UCP}{short = UCP ,long = unresolvable collision pattern}
% V
% W
% X
% Y
% Z


==> tex/displaynotation.tex <==

\cleardoublepage

\section*{Notation}


\bigskip

\begin{center}
\begin{tabular}{ l l l}
\hline \hline
$\load$ & \verb;\load; & Load \\
$\thr$ & \verb;\thr; & Load Threshold\\
$\tp$ & \verb;\tp; & Throughput \\
$\rate$ & \verb;\rate; & Average Rate (inverse of average repetition degree)\\
$\ind$ & \verb;\ind; & Index of the Degree Distributions \\
$\ld$ & \verb;\ld; & Burst Node Degree Distribution, edge-oriented, $\ld(\x)$ \\
$\EBdegDist$ & \verb;\EBdegDist; & Edge Burst Node Degree Distribution\\
$\Ld$ & \verb;\Ld; & Burst Node Degree Distribution, node-oriented, $\Ld(\x)$
 \\
$\BNdegDist$ & \verb;\BNdegDist; & Burst Node Degree Distribution\\
$\davg$ & \verb;\davg; & Average Repetition Degree \\
$\dmax$ & \verb;\dmax; & Maximum Repetition Degree \\
$\rd$ & \verb;\rd; & Slot Node Degree Distribution, edge-oriented, $\rd(\x)$ \\
$\ESdegDist$ & \verb;\ESdegDist; & Edge Sum Node Degree Distribution\\
$\Rd$ & \verb;\Rd; & Slot Node Degree Distribution, node-oriented, $\Rd(\x)$ \\
$\SNdegDist$ & \verb;\SNdegDist; & Slot Node Degree Distribution\\
$\exitb$ & \verb;\exitb; & Burst Node EXIT function, $\exitb(\p)$ \\
$\exits$ & \verb;\exits; & Slot Node EXIT function, $\exits(\q)$ \\
$\area$ & \verb;\area; & Area (general)\\
$\areab$ & \verb;\areab; & Area under the Burst Node EXIT function\\
$\areas$ & \verb;\areas; & Area under the Slot Node EXIT function\\
$\plos$ & \verb;\plos; & Burst loss probability (after decoding)\\
$\plostarget$ & \verb;\plostarget; & Target burst loss probability (after decoding)\\
$\x$ & \verb;\x; & x as dummy variable\\
$\p$ & \verb;\p; & Erasure probability at the output of a Slot Node (average)\\
$\q$ & \verb;\q; & Erasure probability at the output of a Burst Node (average)\\
$\qtarget$ & \verb;\qtarget; & Target erasure probability at the output of a Burst Node\\
\hline \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{ l l l}
\hline \hline
$\snr$ & \verb;\snr; & Instantaneous Signal-to-Noise Ratio\\
$\snrrv$ & \verb;\snrrv; & Signal-to-Noise Ratio Random Variable\\
$\snravg$ & \verb;\snravg; & Average Signal-to-Noise Ratio\\
$\snrdist$ & \verb;\snrdist; & Signal-to-Noise Ratio Distribution, $\snrdist(\snr)$\\
$\snrthr$ & \verb;\snrthr; & Decoding Threshold\\
$\power$ & \verb;\power; & Instantaneous Signal Power\\
$\poweravg$ & \verb;\poweravg; & Average Signal Power\\
$\powerrv$ & \verb;\powerrv; & Signal Power Random Variable\\
$\powerdist$ & \verb;\powerdist; & Signal Power Distribution, $\powerdist(\power)$\\
$\noise$ & \verb;\noise; & Noise Power\\
$\fail$ & \verb;\fail; & Decoding Failure Event\\
$\de$ & \verb;\de; & Differential Operator\\

\hline \hline
\end{tabular}
\end{center}











\clearpage

